CAKE: Sharing Slices of Confidential Data on Blockchain

Cooperative information systems typically involve various entities in a collaborative process within a distributed environment. Blockchain technology offers a mechanism for automating such processes, even when only partial trust exists among participants. The data stored on the blockchain is replicated across all nodes in the network, ensuring accessibility to all participants. While this aspect facilitates traceability, integrity, and persistence, it poses challenges for adopting public blockchains in enterprise settings due to confidentiality issues. In this paper, we present a software tool named Control Access via Key Encryption (CAKE), designed to ensure data confidentiality in scenarios involving public blockchains. After outlining its core components and functionalities, we showcase the application of CAKE in the context of a real-world cyber-security project within the logistics domain.

==> sections/briearchitecture.tex <==
\begin{figure}[h]
	\includegraphics[width=\textwidth]{BRIEarchitecture}
	\caption{BRIE project architecture}
	\label{fig:brie:architecture}
\end{figure}

\todo[inline]{Here I would have expected the CAKE architecture, not the BRIE architecture. And in the BRIE architecture, the interconnecting SPECK module is necessary. Otherwise, it is not correct.}

\Cref{fig:brie:architecture} shows the architecture of the BRIE project solution. It is composed by a front-end module that delivers the BRIE platform's services to the users. It shows data to users and manages the associated processes and documents. Its key functionalities include facilitating the viewing and creation flow of practices and implementing the data clean room feature. The latter displays the system data in an anonymized and aggregated manner, providing users with an overview without disclosing sensitive information.

The back-end constitutes the system component responsible for collecting and managing data pertaining to practices. Additionally, it oversees the authentication process, ensuring that actions are exclusively performed by authorized users. Regarding the data clean room visualization, the back-end module aggregates practice data to provide anonymized insights to the front-end. 
The documents are handled in a draft state, after which they are sent through the CAKE module to IPFS and Algorand for certification.

The CAKE module is responsible for the interaction between the BRIE system and the Algorand blockchain as well as the IPFS network. CAKE exposes REST APIs that allow the back-end to asynchronously send documents for certification. The document upload process is implemented as depicted in \cref{fig:brie:writingflow}.

\begin{figure}[h]
	\includegraphics[width=.65\textwidth]{writing flow}
	\caption{Writing flow of the system}
	\label{fig:brie:writingflow}
\end{figure}

Via the first API endpoint (1), the back-end communicates with the BRIE system to specify the involved actors in the process, thereby granting them access to the uploaded document. Following this, the CAKE system generates a novel \texttt{process ID} and encrypts a file incorporating the role mapping provided by the back-end. Subsequently, this encrypted file is uploaded to IPFS, while on the Algorand blockchain is stored the process ID alongside a reference to the previously uploaded IPFS file. Finally, the process ID is returned to the back-end for storage.

Upon receiving the process ID, the data owner initiates a handshake call (2) to the CAKE module, signaling the intention to upload a document associated with a specific process ID. In response, the data owner obtains a unique identifier known as the \texttt{handshake ID}. Using both the handshake ID and the process ID, the data owner proceeds to transmit the document (3) for encryption while specifying the access policies that delineate the authorized participants within the process who may access the document. The CAKE system employs Attribute Based Encryption (ABE) to encrypt the document before uploading it to IPFS and the obtained resource locator to the Algorand blockchain alongside a unique identifier called \texttt{message ID}. Each document can be divided into distinct parts referred to as \texttt{slices}, with each slice being assigned a unique access policy.

For the file accessing phase, the reader makes a request through the back-end to the CAKE module as shown in \cref{fig:brie:readingflow}.

\begin{figure}[h]
	\includegraphics[width=.65\textwidth]{reading flow}
	\caption{Reading flow of the system}
	\label{fig:brie:readingflow}
\end{figure}

The first step (1) of the client to request to access a document involves an handshake operation in which it communicates to the CAKE module its blockchain address and the process ID it intends to access. Subsequently, the CAKE module provides a unique identifier for the handshake.

At this stage, the back-end can request the generation of a key (2) for the specific process ID. The CAKE system then verifies the attributes associated with the requested process ID. This involves retrieving the encrypted file previously created during the writing process from IPFS, obtaining its reference stored in the Algorand blockchain. The CAKE module produces a decryption key which is based on the attributes retrieved from the IPFS file. This key ensures that the requester indeed has the authorization to access a particular document.

The final step involves the request for accessing data (3). Using the key generated, the CAKE system attempts to access the document stored on IPFS obtaining its resource locator from the blockchain using the message ID sent by the user. If the requester is authorized to access the document, the requested data is returned.
